Dark Energy Survey Year 3 results: Magnification modeling and impact on cosmological constraints from galaxy clustering and galaxy-galaxy lensing

We study the effect of magnification in the Dark Energy Survey Year 3 analysis of galaxy clustering and galaxy-galaxy lensing, using two different lens samples: a sample of Luminous red galaxies, redMaGiC, and a sample with a redshift-dependent magnitude limit, MagLim. We account for the effect of magnification on both the flux and size selection of galaxies, accounting for systematic effects using the Balrog image simulations. We estimate the impact of magnification on the galaxy clustering and galaxy-galaxy lensing cosmology analysis, finding it to be a significant systematic for the MagLim sample. We show cosmological constraints from the galaxy clustering auto-correlation and galaxy-galaxy lensing signal with different magnifications priors, finding broad consistency in cosmological parameters in $\Lambda$CDM and $w$CDM. However, when magnification bias amplitude is allowed to be free, we find the two-point correlations functions prefer a different amplitude to the fiducial input derived from the image simulations. We validate the magnification analysis by comparing the cross-clustering between lens bins with the prediction from the baseline analysis, which uses only the auto-correlation of the lens bins, indicating systematics other than magnification may be the cause of the discrepancy. We show adding the cross-clustering between lens redshift bins to the fit significantly improves the constraints on lens magnification parameters and allows uninformative priors to be used on magnification coefficients, without any loss of constraining power or prior volume concerns.

==> scratch.tex <==
%place to put scraps of text we might want to do something with later

\begin{comment}
When applying a constant $\kappa$ to an image, the effect produced by magnification is that galaxies will get larger.  We would like to know exactly how the size of the galaxies changes when a constant convergence field is applied. From Eq.~(\ref{eq:surface_brightness}), we find that the change in area of a galaxy is:
\begin{equation}
    A^\text{obs}_\text{gal} = \mu  A^\text{int}_\text{gal} 
\end{equation}
Assuming an elliptical shape, the area of the galaxy is:
\begin{equation}
    A^\text{int}_\text{gal} = \pi\, a\, b
\end{equation}
Thus, together with Eq.~(\ref{eq:magnification_kappa}) the magnified galaxy will have the following area: 
\begin{equation}
    A^\text{obs}_\text{gal} = \pi  \, a\, b\, \mu = \pi  (a\sqrt{\mu})\, (b\sqrt{\mu})= \pi  (a\sqrt{1+2\kappa})\, (b\sqrt{1+2\kappa}).  
\end{equation}

Therefore, applying a constant $\kappa$ to an image is equivalent to increasing the length of each galaxy semi-axis by a factor of $f_l=\sqrt{1+2\kappa}$. For instance, if $\kappa=0.01$, $f_l \approx 1.010$ (1\% increase) and if $\kappa = 0.1$, $f_l \approx 1.095$ (9.5\% increase).  
\end{comment}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Estimating Balrog uncertainty}

Estimator of $C_{\text{flux}}$,

\begin{equation} \label{eqn:estimator}
    \hat C_{\text{flux}} =  \frac{N_{o}-N_{i}}{N_{i} \delta\kappa} =\frac{\Delta N}{N_{i} \delta\kappa}.
\end{equation}

Assuming $N_{o{\bar i}}~>>~N_{{\bar o}i}$ we can assume $N$ and $\Delta N$ are independent Poisson fields. The fraction uncertainty in $C$,
\begin{equation}
    \frac{\sigma_{C}}{C} = \sqrt{ \Big[ \frac{1}{\Delta N} + \frac{1}{N_{i}}\Big] }
\end{equation}

sub in Eqn.~\ref{eqn:estimator}, 
\begin{equation}
    \frac{\sigma_{C}}{C} = \sqrt{\frac{1+C\delta\kappa}{C\delta\kappa N}}
\end{equation}

Lets say we want to modify the galaxy length by $1\%$ so $\delta \kappa=0.01$. The estimated $C_{\text{flux}}$ from the luminosity function was $\sim2$. 
%If $N_{i}~>>~\Delta N$ we can approximate this as,

If we do not want to assume $N_{o{\bar i}}~>>~N_{{\bar o}i}$, then the fractional uncertainty can we written as,

\begin{equation}
    \frac{\sigma_{C}}{C} = \sqrt{ \frac{ N_{o{\bar i}}+ N_{{\bar o}i}}{\Delta N^{2}} + \frac{1}{N_{i}} + \frac{2 N_{{\bar o}i}}{\Delta N N_{i}} }
\end{equation}


\begin{equation}
    \frac{\sigma_{C}}{C} = \frac{7.1}{\sqrt{N}}
\end{equation}

so for a $10\%$ statistical error we would need $\sim5000$ balrog lenses, for a $1\%$ statistical error on $C_{\text{flux}}$ we would need $\sim500000$ balrog lenses. Applying a larger $\kappa$ would increase the size of the effect and reduce the required number of lenses.  For instance, if we applied $\delta\kappa=0.02$ we would need $>2600$ balrog lenses per lens bin at $ 10\%$ precision. 

If there is noise in the photometry fitting (e.g. the initialisation noise in mof/sof), some galaxies might exit the sample when magnification is applied, as well as exit. Define, $N_n$ as number of objects in sample with no magnification, $N_m$ number of objects in sample with magnification, $N_{\rm in}$ objects magnification sample but not no magnification sample,  $N_{\rm out}$ objects in no magnification sample but not in magnification sample, $N_{\rm both}$ objects in both. 

\begin{eqnarray}
    N_n = N_{\rm both} + N_{\rm out}
    N_m = N_{\rm both} + N_{\rm in}
    \Delta N = N_{\rm in} - N_{\rm out}
\end{eqnarray}

One can show the error on $C_{\rm flux}$ in this case is 

\begin{equation}
    \sigma_C = C \sqrt{ \frac{N_{\rm in}+ N_{\rm out}}{\Delta N^{2}} + \frac{1}{N_n} + \frac{2 N_{\rm out}}{\Delta N N_n}  }
\end{equation}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Separating magnification effects}

The two effects of magnification, the area and flux effects, can be explored independently. 

\subsubsection{Area}

The solid angle effect modifies the overdensity by,

\begin{equation}\label{eq:delta_mag_area}
   1+\delta_g^{\text{mag, area}}(F) = (1-2\kappa)\, \frac{n^\text{int}\left(F\right)}{n^\text{int}(F)}.
\end{equation}
This implies $C=-2$ for the area effect only.

\subsubsection{Flux}

The flux effect modifies the overdensity by,

\begin{equation}\label{eq:delta_mag_flux}
   1+\delta_g^{\text{mag, flux}}(F) =  \frac{n^\text{int}\left(F-2\kappa F\right)}{n^\text{int}(F)}.
\end{equation}

Following the method of arXiv:1611.10326, we can parameterize the number counts by,

\begin{equation}\label{eq:n_model}
   n^\text{int}(F) = A \left( \frac{F}{F_{*}} \right)^{\alpha(F)}  
\end{equation}
where $A$ and $F_{*}$ are constants and $\alpha$ is a function of the flux limit. We can sub Eqn. \ref{eq:n_model} into Eqn. \ref{eq:delta_mag_flux} to get, 

\begin{equation}\label{eq:delta_mag_flux2}
   \delta_g^{\text{mag, flux}}(F) = \mu^{-\alpha(F)} - 1 
\end{equation}

(\textcolor{red}{I think they assume $F\mu = F(1+2\kappa) \approx F$ in the numerator? not sure about this step.})

Expand and convert to magnitudes,

\begin{equation}\label{eq:delta_mag_flux2}
   \delta_g^{\text{mag, flux}}(F) = 2\alpha(m)\kappa, 
\end{equation}

where,

\begin{equation}\label{eq:delta_mag_flux2}
   \alpha = 2.5\frac{d}{dm}[\log{n^\text{obs}(m)}].
\end{equation}

The flux effect has $C=2\alpha(m)$ if assuming this model (ideal flux limited sample\textcolor{red}{?}). 

\subsubsection{Area and Flux}

Including both effects at the same time, the effects on $\delta_g^{\text{mag}}$ are additive to first order,

\begin{equation}\label{eq:delta_mag_flux2}
   \delta_g^{\text{mag}}(F) = 2[\alpha(m)-1]\kappa. 
\end{equation}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{comment}
For a galaxy at some distance $d$, a square patch with side length $D$ subtends an angle $\alpha = D/d$ on the sky. Assuming this patch has an intrinsic luminosity $L$, the total flux we see is 

\begin{equation}
 F = \frac{L}{$4\pi d^2$}.   
\end{equation}

2nd law of theromodyanamics. 

 Also note that light is neither created nor destroyed by lensing, just redistributed. That means that if you see increased fluxed due to lensing, some other observer with a different line of sight would have to see diminished flux to compensate.
  
The surface brightness is independent of distance (to first order). This is because the flux coming from an object decreases as $1/d^2$ for an object is located at distance d, while the solid angle subtended by the object decreases also as $1/d^2$. Thus the surface brightness at a given point on the surface of the galaxy is a well-defined distance-independent quantity. 

Since photons are neither emitted nor absorbed in the process of gravitational light deflection, the surface brightness of lensed sources remains unchanged. 


\end{comment}

==> theory_old.tex <==
\section{Theory}
\label{sec:theory}

\subsection{Modeling the correlation functions}

The modeling of the two point functions is described in detail in \cite{y3-generalmethods}. In this section we outline the basic structure of this model, before describing the magnification contribution in detail. 

For all of the angular power spectra apart from the galaxy clustering spectrum we use the Limber approximation, 
 \begin{align}
     \label{eq:cl}
     C_{AB}^{ij}(\ell) = \int d\chi \frac{W_A^i(\chi)W_B^j(\chi)}{\chi^2}P_{AB}\left(k = \frac{\ell+0.5}{\chi},z(\chi)\right)\,,
 \end{align}
 
where ......
 
The Limber approximation is insufficient for computing the angular clustering power spectrum, and we follow the \cite{Fang_nonlimber} in evaluating angular power spectra without the Limber approximation. For example, the exact expression for the density-density contribution to the angular clustering power spectrum is
\begin{align}
  \nonumber   C_{\delta_{g,\rm D}\delta_{g,\rm D}}^{ij} (\ell)=&\frac{2}{\pi}\int d \chi_1\,W^i_{\delta,{g}}(\chi_1)\int d\chi_2\,W^j_{\delta,g}(\chi_2)\\
     &\int\frac{dk}{k}k^3 P_{gg}(k,\chi_1,\chi_2)j_\ell(k\chi_1)j_\ell(k\chi_2)\,,
 \label{eq:Cl_DD}
\end{align}
and the full expressions including magnification and redshift-space distortion are given in \cite{Fang_nonlimber}. Schematically, the integrand in Eq.~\ref{eq:Cl_DD} is split into the contribution from non-linear evolution, for which un-equal time contributions are negligible so that the Limber approximation is sufficient, and the linear-evolution power spectrum, for which time evolution factorizes. \footnote{\url{https://github.com/xfangcosmo/FFTLog-and-beyond}} developed in \cite{Fang_nonlimber} to evaluate the full angular clustering power spectrum, including magnification and redshift-space distortion contributions.
 

We relate the power spectra to the angular correction functions with,
\begin{align}
    w^i(\theta) =& \sum_\ell \frac{2\ell+1}{4\pi}P_\ell(\cos\theta) C^{ii}_{\delta_{\mathrm{l,obs}}\delta_{\mathrm{l,obs}}}(\ell)~,\\
    \gamma_t^{ij}(\theta) =& \sum_\ell \frac{2\ell+1}{4\pi\ell(\ell+1)}P^2_\ell(\cos\theta) C^{ij}_{\delta_{\mathrm{l,obs}}\mathrm{E}}(\ell)~,
\end{align}
where $P_\ell$ and $P_\ell^2$ are the Legendre polynomials. 

\subsection{Magnification}
\label{sec:magnification_theory}

We can express magnification as the determinant of the inverse of the Jacobian matrix $\mathcal{A}$, and in terms of the convergence $\kappa$ and the shear $\gamma$:
\begin{equation}\label{eq:magnification_kappa}
    \mu = \frac{1}{det \mathcal{A}} = \frac{1}{(1-\kappa)^2 - \vert \gamma \vert ^2 } \approx \frac{1}{1-2\kappa}\approx 1+ 2\kappa,
\end{equation}
in the limit of weak lensing when $\kappa \ll 1$ and $\gamma \ll 1$. 

Magnification can alter the local number density of galaxies due to two different reasons: 
\begin{itemize}
    \item \textbf{Increase of area}: For a fixed set of sources, the number density of images decreases by a factor $\mu$ as the sky is locally stretched. 
    \item \textbf{Increased flux of individual galaxies}: Since lensing conserves surface brightness, magnification increases the size of galaxy images at a fixed surface-brightness level. The resulting flux enhancement enables galaxies to be seen down to fainter intrinsic magnitudes, and consequently the local number density of galaxies observed in images above a certain flux threshold can be altered by lensing. 
\end{itemize}

Whether the first, purely geometrical dilution effect wins over the second, astrophysical effect depends on the intrinsic slope of the cumulative flux distribution. The larger the ratio of faint to bright objects in the sample, the steeper the distribution, and the stronger is the number density increase.

The overdensity due to magnification is the ratio between the observed number density and the intrinsic number density that we would obtain without magnification:
\begin{equation}
    \label{eq:delta_mag_flux}
    1+\delta_g^{\text{mag}}(F,\vec{\theta}) = \frac{ n^\text{obs}(F,\vec{\theta}) }{ n^\text{int}(F,\vec{\theta}) }
\end{equation}

Putting the two effects produced by magnification described above together we can express the observed number density of galaxies in a redshift slice with flux within $dF$ of $F$ and direction in the sky $\vec{\theta}$ as:
\begin{equation}
    n^\text{obs}(F,\vec{\theta}) = \frac{1}{\mu(\vec{\theta})} n^\text{int}(F/\mu(\vec{\theta}), \vec{\theta}).
\end{equation}

Therefore, in order to find the increase in number density due to magnification, we will need to measure the relation between $n^\text{int}(F)$ and $n^\text{int}(F/\mu)$:
\begin{equation}
   1+\delta_g^{\text{mag}}(F, \vec{\theta}) = \frac{1}{\mu(\vec{\theta})} \frac{n^\text{int}(F/\mu(\vec{\theta}), \vec{\theta})}{n^\text{int}(F, \vec{\theta})}.
\end{equation}

Dropping the dependency on angular position and using Eq.~(\ref{eq:magnification_kappa}), we can also express the change in number density as a function of convergence:
\begin{equation}\label{eq:delta_mag}
   1+\delta_g^{\text{mag}}(F) = (1-2\kappa)\, \frac{n^\text{int}\left((1-2\kappa)\, F\right)}{n^\text{int}(F)}.
\end{equation}

Under idealised conditions, it can be shown (e.g. in \cite{sv-magnification}) that one can approximate this as, 

\begin{equation}\label{eq:delta_mag_alpha}
   \delta_g^{\text{mag}}(F) = 2[\alpha(m)-1]\kappa. 
\end{equation}

where $\alpha$ is the slope of the intrinsic flux distribution
\begin{equation}\label{eq:alpha}
   \alpha = 2.5\frac{d}{dm}[\log{n^\text{obs}(m)}].
\end{equation}

We will write the $2[\alpha(m)-1]$ prefactor as a constant $C=\csample+\carea$ where $\carea=-2$ captures the increase in area affect, and $\csample$ is a constant to be determined. This constant is equal to $2\alpha$ in the idealised case when the sample in question has a constant flux limit and no other selection effects. 


\subsection{Lens magnification}

The primary affect we will study is magnification of the lens sample by structure that is between the lenses and the observer. We can express the observed density contrast for the lens sample as:
\begin{equation}
    \delta_g^\text{obs} =  \delta_g^\text{int} + \delta_g^\text{mag}.
\end{equation}

Following Section  \ref{sec:magnification_theory}, we can write the change in number density produced by magnification as proportional to the convergence, and we define $C$ as: 
\begin{equation}\label{eq:definition_C}
\delta_g^\text{mag} (\theta) = C \kappa_l (\theta)
\end{equation}

Then, this change in the density contrast affects both galaxy-galaxy correlations:
\begin{equation}
\left< \delta_g^\text{obs} \delta_g^\text{obs} \right> = \left< \delta_g^\text{int} \delta_g^\text{int} \right>  + C^2\left< \kappa_l\kappa_l \right> + 2C \left< \delta_g^\text{int} \kappa_l \right> ,
\end{equation}
and galaxy-shear correlations:
\begin{equation}
\left< \delta_g^\text{obs} \gamma \right> = \left< \delta_g^\text{int} \gamma \right> + C\left< \kappa_l\gamma \right> = \left< \delta_g^\text{int} \gamma \right> + C\left< \kappa_l\kappa_s \right>,
\end{equation}
since $\gamma \propto \kappa$. 

The $\langle \kappa \kappa \rangle$ terms are computed in Fourier space using Eqn. \ref{eq:cl} and are added to the clustering and galaxy-galaxy lensing $C(l)$ before projecting into the real space correlation functions.  


\begin{comment}
\subsection{Lens magnification and reduced shear}

We can also consider the effect of reduced shear, which only affects the galaxy-shear correlations. Reduced shear changes the observed shear by the following factor: 
\begin{equation}\label{eq:reduced_shear}
    \gamma^{\text{obs}} =  \gamma^{\text{int}} (1 + \kappa_s),
\end{equation}
where $\kappa_s$ is the convergence field at the redshift of the source galaxies. On the other hand, we have seen above that the observed number density of lens galaxies changes because of lens magnification in the following way: 
\begin{equation}\label{eq:delta_g_obs}
      \delta_g^\text{obs} =  \delta_g^\text{int} + \delta_g^\text{mag} =  \delta_g^\text{int} +  C \kappa_l,
\end{equation}
using the parametrization from Eq.(\ref{eq:definition_C}) and where $\kappa_l$ is the convergence field at the redshift of the lens galaxies. Thus, putting the two effects together, the galaxy-galaxy lensing correlations between lens galaxy positions and source galaxy shears are:
\begin{equation}
\begin{split}
   \left< \delta_g^\text{obs} \gamma \right> &= \left< (\delta_g^\text{int} +  C \kappa_l) \,  \gamma^{\text{int}} \, (1 + \kappa_s) \right> =  \\
   &=  \underbrace{\left< \delta_g^\text{int} \gamma^{\text{int}}\right>}_{\text{signal}} +  \underbrace{\left< \delta_g^\text{int}\gamma^{\text{int}} \kappa_s \right>}_{\text{reduced shear}} + \, \underbrace{C\left< \gamma^{\text{int}}\kappa_l \right>}_{\text{lens mag}} + \, \underbrace{C\left< \gamma^{\text{int}}\kappa_l \, \kappa_s \right>}_{\text{reduced shear + lens mag}},
   \end{split}
\end{equation}

where the first term is the pure galaxy-shear signal, the second term contains the effect of reduced shear only, the third term contains the effect of lens magnification only and the last term has corrections from both reduced shear and lens magnification. 

\subsection{Lens magnification, reduced shear, source magnification and source clustering}

We can also consider the effect of source magnification and source clustering, which also only affects the galaxy-shear correlations. On top of the previously mentioned effects, these change the observed shear by the following factors: 
\begin{equation}\label{eq:gamma_obs_full}
    \gamma^{\text{obs}} =  \gamma^{\text{int}} (1 + \kappa_s) (1 + \delta_s + C_s \kappa_s),
\end{equation}
where $\delta_s$ includes the effect of source clustering and $C_s \kappa_s$ the effect of source magnification. Cross-correlating the expression above with Eq.~(\ref{eq:delta_g_obs}) and now labeling the lens galaxy density as $\delta_l$  to distinguish it from the source galaxy density, we obtain:
\begin{equation}
\begin{split}
 \left< \delta_l^\text{obs} \gamma \right> &= \left< (\delta_l^\text{int} +  C_l \kappa_l) \,  \gamma^{\text{int}} \, (1 + \kappa_s) (1 + \delta_s + C_s \kappa_s)\right> =  \\
 &= \underbrace{\left< \delta_l^\text{int} \gamma^{\text{int}}\right>}_{\text{signal}}  
 + \, \underbrace{C_l\left< \gamma^{\text{int}}\kappa_l \right>}_{\text{lens mag}} + \,
\underbrace{ (1+ C_s) \left< \delta_l \, \gamma^{\text{int}} \kappa_s \right> }_\text{source mag + reduced shear} + \\
&+ \underbrace{ C_l \, (1+ C_s) \left<  \gamma^{\text{int}} \kappa_s \kappa_l \right> }_\text{lens mag + source mag + reduced shear} +
\underbrace{ C_l  \left< \delta_s \gamma^{\text{int}} \kappa_l \right> }_\text{lens mag + source clustering}
   \end{split}
\end{equation}

\subsection{Source magnification}
We can also consider the effect of source magnification, which will affect the galaxy-shear cross-correlations and the shear-shear autocorrelation.  

\begin{equation}\label{eq:gamma_obs_full}
    \gamma^{\text{obs}} =  \gamma^{\text{int}} (1 + C_s \kappa_s),
\end{equation}
where $C_s \kappa_s$ characterizes the effect of source magnification on the source sample. 

\section{Effect of magnification to boost factors}

\begin{equation}
    \delta_g^\text{obs} =  \delta_g^\text{int} + \delta_g^\text{mag} 
\end{equation}

\begin{equation}
    \delta_s^\text{obs} =  \delta_s^\text{int} + \delta_s^\text{mag} 
\end{equation}

\begin{equation}
C_l \kappa_l(\theta)
\end{equation}

\begin{equation}
C_s \kappa_s(\theta)
\end{equation}


We estimate the boost factors like this: 
\begin{equation}
    B(\theta) = \frac{N_r}{N_l}  \frac{\sum_{l,s} w_{l,s}}{\sum_{r,s}w_{r,s}}
\end{equation}
And thus it has the form of a clustering correlation function. Then:
\begin{equation}
\left< \delta_g^\text{obs} \delta_s^\text{obs} \right> = \left< \delta_g^\text{int} \delta_s^\text{int} \right>  + C_l\,  C_s\left< \kappa_l \kappa_s \right> + C_l \left< \kappa_l \delta_s^\text{int}  \right>  + C_s \left< \delta_l^\text{int} \kappa_s \right>,
\end{equation}

\end{comment}
